A Pattern Language for Machine Learning Tasks

We formalise the essential data of objective functions as equality constraints on composites of learners. We call these constraints "tasks", and we investigate the idealised view that such tasks determine model behaviours. We develop a flowchart-like graphical mathematics for tasks that allows us to; (1) offer a unified perspective of approaches in machine learning across domains; (2) design and optimise desired behaviours model-agnostically; and (3) import insights from theoretical computer science into practical machine learning. As a proof-of-concept of the potential practical impact of our theoretical framework, we exhibit and implement a novel "manipulator" task that minimally edits input data to have a desired attribute. Our model-agnostic approach achieves this end-to-end, and without the need for custom architectures, adversarial training, random sampling, or interventions on the data, hence enabling capable, small-scale, and training-stable models.

==> sections/A1-CompManipulator.tex <==
\section{Complement \texttt{Manipulation}}
\label{appendix:compMan}
\begin{minipage}{\textwidth}
    \begin{minipage}{0.5\textwidth}
        \begin{pattern}[\texttt{complement manipulation}]\label{patt:compManipulator}
        \[\tikzfig{manipulatorComp}\]
        \end{pattern}
    \end{minipage}
    \begin{minipage}{0.5\textwidth}
        Let $\mathcal{X}: (d, \textcolor{cbblue}{a})$ be a distribution over some data $d \in D$, each labelled with an attribute $\textcolor{cbblue}{a} \in \textcolor{cbblue}{A}$. A \texttt{complement manipulator} consists of a pair ($\texttt{get}: D \to \textcolor{cbblue}{A}$, $\overline{\texttt{put}}: D \otimes \textcolor{cbblue}{A} \otimes \textcolor{cborange}{C} \to \mathcal{D} \otimes \textcolor{cborange}{C}$) fulfilling the rules on the left. The idea of the complement is that it provides the {manipulator} with a scratchpad $C$ to record whatever it needs in order to translate between non-bijective distributions without steganography. In fact, none of the tasks ever check the output of the complement, therefore no requirements are made for it at all. \autoref{sec:exp-spriteworld} shows this definition of the {manipulator} in action. This solution is similar to the proposal in the conclusion of \citep{chu2017cyclegan}, the paper which originally observed this challenge for {CycleGANs}; they propose introducing a complement to add to the distribution with lower entropy.
    \end{minipage}
\end{minipage}


==> sections/A1-Theory-Proofs.tex <==
\section{Deferred proofs}


% \subsection{Proof of \autoref{prop:energ}}\label{proof:energ}
% \begin{lemma}\label{lem:lincomb}
% For all well-typed $f$, $g$, and for any positive linear combination $\alpha: \textcolor{cbgreen}{\mathbb{R}^{\geq 0}} \times \textcolor{cbgreen}{\mathbb{R}^{\geq 0}} \rightarrow \textcolor{cbgreen}{\mathbb{R}^{\geq 0}}$:
% \[\tikzfig{energy/lem3} \quad \sim \quad \tikzfig{energy/lem2b}\]
% \begin{proof}
% For the forward refinement, as $\alpha$ is a positive linear combination, we have for all $x \in \mathcal{X}$ that $\alpha(f(x), g(x)) = \alpha_1 \cdot f(x) + \alpha_2 \cdot g(x) = \textcolor{cbgreen}{0}$. If $f$ and $g$ are constant-functions $0$, we are done. Otherwise, positivity implies that $\alpha_1 \cdot f(x) = \alpha_2 \cdot g(x) = \textcolor{cbgreen}{0}$, and since $\alpha_1,\alpha_2 \in \textcolor{cbgreen}{\mathbb{R}^{\geq 0}}$, then $f(x) = \textcolor{cbgreen}{0} = g(x)$, which is the desired task. For the backwards refinement, if $f(x) = \textcolor{cbgreen}{0} = g(x)$ for all $x \in \mathcal{X}$, then \mbox{$\alpha(f(x), g(x)) = \alpha_1 \cdot f(x) + \alpha_2 \cdot g(x) = \textcolor{cbgreen}{0}$}.
% \end{proof}
% \end{lemma}

% \begin{lemma}\label{lem:positivity}
% For a real-valued pairwise measure $\mathbf{D}: \mathcal{D}(Y) \times \mathcal{D}(Y) \rightarrow \textcolor{cbgreen}{\mathbb{R}^{\geq 0}}$ on the space of distributions over $Y$, the positivity axiom $\mathbf{D}(\mathcal{Y}_1,\mathcal{Y}_2) = \textcolor{cbgreen}{0} \iff \mathcal{Y}_1 = \mathcal{Y}_2$ implies, for (almost\footnote{When the function space containing $f$ and $g$ is large, the edge case where $f$ and $g$ are nonconstant and $f = -g$ is negligible. Since we are concerned with behaviour in the computational limit, this is an acceptable assumption for our purposes.}) all $f,g : X \rightarrow Y$ and $\mathcal{X}$: 
% \[\tikzfig{energy/lem1b} \quad \sim \quad \tikzfig{energy/lem1}\]
% \begin{proof}
% For the forward refinement, we assume that $\mathbf{D}(f(\mathcal{X},g(\mathcal{X}))) = \textcolor{cbgreen}{0}$. By positivity of $\mathbf{D}$, $f(\mathcal{X}) = g(\mathcal{X})$, which is the right hand task. For the backward refinement, if $f(\mathcal{X}) = g(\mathcal{X})$, then, by positivity, $\mathbf{D}(f(\mathcal{X},g(\mathcal{X}))) = \textcolor{cbgreen}{0}$.
% \end{proof}
% \end{lemma}

% \begin{proposition}
% If \texttt{enc} and \texttt{dec} are deterministic and $\mathbf{E}_{\texttt{enc}}$ and $\mathbf{E}_{\texttt{dec}}$ are positive (e.g. metrics or statistical divergences), then \texttt{energy minimisation} $\equiv$ \texttt{autoencoding}.
% \begin{proof}
% As \texttt{enc} and \texttt{dec} are functions, we may copy them through their outputs to re-express \texttt{energy minimisation} as:
% \[\tikzfig{energy/proof}\]
% By \autoref{lem:lincomb}, this is equivalent to:
% \[\tikzfig{energy/proof1}\]
% Recall that $\mathbf{E}_{\texttt{enc}}$ and $\mathbf{E}_{\texttt{dec}}$ are positive by definition, hence \autoref{lem:positivity} allows us to express the two minimisations as:
% \[\tikzfig{energy/proof2}\]
% The left task is \texttt{autoencoding}, so we have that \texttt{energy minimisation} refines \texttt{autoencoding}. For the other direction, we observe that \texttt{autoencoding} refines the right task by postcomposing both sides with \texttt{enc}, and as the left and right tasks together are equivalent to \texttt{energy minimisation}, we have the claim.
% \end{proof}
% \end{proposition}



\subsection{Proof of \autoref{prop:cyclegan}}\label{apdx:gan}
\texttt{CycleGAN}s (\autoref{task:cycleGAN}) solve a similar task as \texttt{manipulation}, translating between two distributions. In fact, with the additional regularisation terms, \texttt{strong manipulation} (see \autoref{appendix:strong-manipulation}) is a refinement of \texttt{CycleGAN}, giving us more guarantees by avoiding certain failure cases. We can use the pattern language to show this formally. However, in both cases, the tasks are not perfectible, as, by design, it is impossible for the generator and the discriminator to have a loss of zero at the same time. Therefore, we have to generalise the definition of \emph{refinement} for \emph{partially perfectible tasks}.


\begin{defn}[Partially perfectible task]
    A \emph{partially perfectible task} ${\{(f_i,g_i,\mathcal{X}_i, \mathfrak{p}_i)\}_i}$ with learnable functions $\Sigma_l$ is a compound task with excluded learners $E \subseteq \Sigma_l$ such that:
    \begin{enumerate}
        \item no two $e \in E$ share atomic tasks, i.e. $\forall e, e' \in E. \{(f_i,g_i,\mathcal{X}_i, \mathfrak{p}_i) | e \in f_i \lor e \in g_i\} \cap \{(f_i,g_i,\mathcal{X}_i, \mathfrak{p}_i) | e' \in f_i \lor e' \in g_i\} = \emptyset$ and 
        \item all tasks not involving learners from $E$ are perfectible, i.e. $\exists \pi \in \mathfrak{p} . \forall x \in X . f_{i; \pi}(x) = g_{i; \pi}(x)$
    \end{enumerate}
\end{defn}

Importantly, there does not need to exist a perfect solution for all tasks. As condition (1) explicitly forbids excluded learners to share tasks, we do not need to make restrictions on their composite behaviour. An example of a partially perfectible task is \texttt{CycleGAN} with excluded learners $\texttt{dsc}_1, \texttt{dsc}_2$. Assuming an appropriate data distribution \citep{wu2024stegogan}, the \texttt{autoencoding} tasks, i.e. the reconstruction losses, are perfectible. However, the generator-discriminator tasks are not. \texttt{GAN} with excluded learner \texttt{dsc} is another example of a partially perfectible tasks. In this case no tasks are required to be perfectible, as all of them involve the discriminator. 

When we have partially perfectible tasks, we have to define what we mean by an optimal solution. 

\begin{defn}[Optimal partially pefect solution]
    Let $\Phi = {\{(f_i,g_i,\mathcal{X}_i, \mathfrak{p}_i)\}_i}$ be a partially perfectible tasks with learners $\Sigma$ and excluded learners $E \subseteq \Sigma$. Then an \emph{optimal partially perfect solution} for the learners $L = \Sigma \setminus E$ is, if it exists, a set of parameters $\pi_L \in \mathfrak{p}_L$ such that for all $\alpha_L, \mathbf{D}_\phi$ they perfect the perfectible tasks: 
    \[\forall \{(f_i,g_i,\mathcal{X}_i, \mathfrak{p}_i) \in \Phi | \forall e \in E . e \not\in f_i \land e \not\in g_i\}. \forall x \in \mathcal{X}_i . f_{i; \pi_L}(x) = g_{i; \pi_L}(x)\]
    and for all $l \in L$ and all tasks $\Phi_l$ with $\text{para}(l) \cap \mathfrak{p}_i \not= \emptyset$:
    \[\alpha_l(\{\mathop{\mathbb{E}}\limits_{x \sim \mathcal{X}_i}(\textbf{D}_\phi(\text{sys}_{\phi; (\pi_L \cup \mathfrak{p}_E(\pi_L))}(x), \text{spec}_{\phi; \pi_L \cup \mathfrak{p}_E(\pi_L)}(x))) \, | \, \phi \in \Phi_l\})\]
    is minimal over all possible parameter combinations, where \[{\mathfrak{p}_E(\pi_L) = \mathop{\bigcup}\limits_{e \in E} \mathop{\inf}\limits_{\pi_e \in \mathfrak{p}_e} (\alpha_e(\{\mathop{\mathbb{E}}\limits_{x \sim \mathcal{X}_i}(\textbf{D}_\psi(\text{sys}_{\psi; (\pi_L \cup \pi_e)}(x), \text{spec}_{\psi; (\pi_L \cup \pi_e)}(x))) \, | \, \psi \in \Phi_e\}))}\]
\end{defn}
In words, we consider a set of parameters \emph{optimal partially perfect}, if they are perfect for the perfectible tasks and have a minimal objective function for the non-perfectible tasks, even if the excluded learners only optimise for themselves. This may not always exist, either because there is no solution that is optimal for all $\alpha_L, \mathbf{D}_\phi$ or as there may be more optimal solutions for the non-perfectible tasks that do not satisfy the perfectible tasks. 

Given this, we can generalise the definition of \emph{refinement} for partially perfectible tasks. 

\begin{defn}[Optimal refinement of partially-perfectible tasks]
    Given two partially-perfectible tasks $\Psi, \Phi$ with excluded learners $E_\Psi, E_\Phi$, we say that $\Psi$ optimally refines $\Phi$ if optimal partially perfect solutions for $\Sigma_{l_\Psi} \setminus E_\Psi$ can be composed to form optimal partially perfect solutions for $\Sigma_{l_\Phi} \setminus A_\Phi$.
\end{defn}

For $A_\Psi, A_\Phi = \emptyset$, optimal refinement is equivalent to refinement.

To show that \texttt{manipulation} optimally refines \texttt{CycleGAN}, we need one assumption: we assume that the measure of statistical divergence and compound function have been chosen such that a generator in a generative-adversarial setting is optimal if and only if its output distribution is equal to the original distribution. As the goal of such a generative setting is to approximate the original distribution, this is quite a natural assumption. One possible choice of measure of statistical divergence and compound function is given by Goodfellow et al. \citep[Theorem~1]{goodfellowGenerativeAdversarialNetworks2014a} and has been proven to fulfil this assumption.

\begin{proposition}[Manipulation vs. Style-transfer]
    Given appropriately chosen measure of statistical divergence and compound functions, \texttt{strong manipulation} with excluded learner \texttt{dsc} optimally refines \texttt{CycleGAN} with excluded learners $\texttt{dsc}_1$, $\texttt{dsc}_2$. 
\begin{proof}
    Let $\mathcal{X}_1, \mathcal{X}_2$ be two distributions over the same type. We create $\mathcal{X} = (x, i)$ for $x \in \mathcal{X}_i$ where the label $i$ indicates the distribution the data point came from. Assuming that we have $(\texttt{get}, \texttt{put}, \texttt{disc})$ that satisfy \texttt{strong manipulation} with an optimal partially perfect \texttt{put}, \texttt{get}, we can construct optimal partially perfect generators $G_1$ and $G_2$ for \texttt{CycleGAN}.
    
    For $i \in {0, 1}, j = 1 - i$, we define: 
    \[\tikzfig{CycleGAN-man-proof/setup}\]

    First, we show that the perfectible tasks are indeed perfected, i.e. that both the autoencoder tasks are fulfilled. We have: 
    \[\tikzfig{CycleGAN-man-proof/proof1}\]

    Next, we will show that these generators are indeed globally optimal. By assumption, a generator is optimal if and only if its output distribution is indistinguishable from the training distribution. Thus, assuming that the components of \texttt{manipulation} are optimal with respect to the generative-adversarial tasks, $\texttt{put}$ output distribution approaches $\mathcal{X} = (x, i)$ for $x \in \mathcal{X}_i$. But by $\textsc{PutGet}$, we have: 
    \[\tikzfig{CycleGAN-man-proof/proof2}\]

    Therefore, by \textsc{Classify}, $G_1$ and $G_2$ can only return values that are akin to values in $\mathcal{X}_1$ and $\mathcal{X}_2$ respectively. As these two labels make up the entirety of $\mathcal{X}$, $G_1$'s and $G_2$'s output distributions are indistinguishable from $\mathcal{X}_1$ and $\mathcal{X}_2$ respectively. Therefore, they are indeed optimal generators for their respective distribution. 
    
    But then we have shown that $G_1$ and $G_2$ are indeed optimal solutions to \texttt{CycleGAN} and therefore that \texttt{manipulation} is a specialisation of \texttt{CycleGAN}\footnote{In \citep{CycleGAN2017}, when doing style transfer, they additionally add the \emph{identity loss} which enforces that generating an image in $X_i$ given an image from $X_1$ should return the identity. This perfectible task is also guaranteed by \texttt{strong manipulation} by \texttt{cls} and \texttt{GetPut}}.
\end{proof}
\end{proposition}

In turn, \texttt{CycleGAN}, however, is not a refinement of \texttt{strong manipulation}. This means there exist solutions to \texttt{CycleGAN}, which violate \texttt{strong manipulation}. In these image translation tasks, we expect the translators to change as little as possible to go from one distribution to the other, i.e. preserving as much information from the original as possible. However, the generators of \texttt{CycleGAN} could, for example, flip the images horizontally. As the \texttt{autoencoder} tasks have an even number of generators on each side, this would be a `perfect solution' to the outlined task, yet not the behaviour we would want or expect. In contrast, the \textsc{PutPut} rule of \texttt{strong manipulation} does not allow this behaviour. As such, \texttt{strong manipulation} gives us more guarantees than \texttt{CycleGAN}. 

Despite the additional guarantees, \texttt{strong manipulation} does not guarantee that it indeed only changes as little as necessary to go from one distribution to the other. This can be seen when considering a limited toy scenario: the data has the four objects \emph{circle}, \emph{square}, \emph{red} and \emph{green}. There is no unique mapping between shapes and colours. Without further information, it is therefore completely impossible to say what it would mean to change as little as possible to go from shapes to colours. When considering this toy scenario, it becomes obvious that, without specifying further restrictions on all remaining attributes, it is impossible to know which mapping is correct. Yet, despite these theoretical concerns, in practice, even \texttt{manipulation} often converges to the desired behaviour, similar to \texttt{CycleGAN}, which has even fewer guarantees.



==> sections/A3-EnergyMin.tex <==
\section{Energy minimisation}

\begin{lemma}\label{lem:lincomb}
For any positive linear combination $\alpha: \mathbb{R}^{\geq 0} \times \mathbb{R}^{\geq 0} \rightarrow \mathbb{R}^{\geq 0}$:
\[\tikzfig{energy/lem3} \quad \sim \quad \tikzfig{energy/lem2b}\]
\begin{proof}
Without loss of generality let $\alpha(-,=) = \alpha_1(-) + \alpha_2(=)$. For the forward simulation we may assume that for all $x$ from $\mathcal{X}$, $\alpha_1(f(x)) + \alpha_2(g(x)) = 0$. This implies that $\alpha_1(f(x)) = \alpha_2(g(x)) = 0$, and since $\alpha_1,\alpha_2 \in \mathbb{R}^{\geq 0}$, then $f(x) = 0 = g(x)$, which is the desired task. For the backwards simulation, if $f(x) = 0 = g(x)$ for all $x$ from $\mathcal{X}$, then evidently $\alpha_1(f(x)) + \alpha_2(g(x)) = 0$.
\end{proof}
\end{lemma}
\begin{lemma}\label{lem:positivity}
For $\mathbf{D}: \mathcal{D}(Y) \times \mathcal{D}Y \rightarrow \mathbb{R}^{\geq 0}$ a real-valued pairwise measure on the space of distributions over $Y$, the positivity axiom $\mathbf{D}(\mathcal{Y}_1,\mathcal{Y}_2) = 0 \iff \mathcal{Y}_1 = \mathcal{Y}_2$ implies, for all $f,g : X \rightarrow Y$ and $\mathcal{X}$:
\[\tikzfig{energy/lem1b} \quad \sim \quad \tikzfig{energy/lem1}\]
\begin{proof}
For the forward simulation, we assume that $\mathbf{D}(f(\mathcal{X},g(\mathcal{X}))) = 0$. By positivity of $\mathbf{D}$, $f(\mathcal{X}) = g(\mathcal{X})$, which is the right hand task. For the backward simulation, if $f(\mathcal{X}) = g(\mathcal{X})$, by positivity $\mathbf{D}(f(\mathcal{X},g(\mathcal{X}))) = 0$.
\end{proof}
\end{lemma}

\begin{proposition}
If $\mathbf{E}_{\texttt{enc}}$ and $\mathbf{E}_{\texttt{dec}}$ are positive (e.g. metrics or statistical divergences), \texttt{(code-extracting) energy minimisation} is equivalent to \texttt{autoencoder}.
\begin{proof}
By the algebraic properties of copy, we can equivalently express \texttt{energy minimisation} as:
\[\tikzfig{energy/proof}\]
By \autoref{lem:lincomb}, we have that the above is equivalent to:
\[\tikzfig{energy/proof1}\]
By the assumption that $\mathbf{E}_{\texttt{enc}}$ and $\mathbf{E}_{\texttt{dec}}$ are positive, \autoref{lem:positivity} allows us to express the two minimisations as their own tasks.
\[\tikzfig{energy/proof2}\]
The task on the right is implied by the \texttt{autoencoder} task on the left, treated as an equation. This yields the claim.
\end{proof}
\end{proposition}


==> sections/AX-category.tex <==
\subsection{Formal semantics}%\label{appendix:category}

The functional effect of the construction below is to extend the category of continuous maps between Euclidean spaces with global elements that behave as probability distributions instead of points. We presume familiarity with symmetric monoidal categories and their graphical calculi \citep{selingerSurveyGraphicalLanguages2010c}.

Let \textbf{CartSp} denote the coloured PROP \citep{yauHigherDimensionalAlgebras2008} of continuous maps between Euclidean spaces, where the tensor product is the cartesian product --- i.e. \textbf{CartSp} is cartesian monoidal.

Let \textbf{BorelStoch} denote the Markov category \citep{choDisintegrationBayesianInversion2019a,fritzSyntheticApproachMarkov2020} of stochastic kernels \citep{panangadenCategoryMarkovKernels1999} between Borel-measurable spaces. Stochastic kernels in particular subsume the continuous maps between Euclidean spaces.

As a Markov category, in the terminology of \citep{fongSupplyingBellsWhistles2019}, \textbf{BorelStoch} supplies cocommutative comonoids. By Fox's theorem \citep{foxCoalgebrasCartesianCategories1976a} cartesian monoidal categories are precisely those isomorphic to their own categories of cocommutative comonoids. Hence there is a (semicartesian) functorial embedding of \textbf{CartSp} into \textbf{BorelStoch} sending $\mathbb{R}^N$ to $\mathbb{R}^N$ (equipped with the usual Borel measure), and continuous maps to deterministic continuous maps. We declare our semantic category to be generated by the image of this embedding along with the probability distributions $\mathcal{X}: \{\star\} \rightarrow \mathbb{R}^N$, where $\{\star\}$ is the singleton monoidal unit of \textbf{BorelStoch}.





==> sections/snippets.tex <==
\bB 
String diagrams are an intuitive formal syntax for algebraic expressions

String diagrams are an in admit a reasoning system which we will utilise throughout this paper. In addition to regular equational reasoning between such alge 

\e

Optionally, we can add more stringent requirements to obtain \texttt{strong manipulation} with additional behavioural guarantees, at the cost of practical difficulties in training (see~\autoref{apdx:gan}). This can be viewed as adding further regularisation.

These results in turn will \textbf{inform testable predictions about the behaviour of \texttt{put}:}
